Omni-sparsity DNN: Fast Sparsity Optimization for On-Device Streaming E2E ASR via Supernet

From wearables to powerful smart devices, modern automatic speech recognition (ASR) models run on a variety of edge devices with different computational budgets. To navigate the Pareto front of model accuracy vs model size, researchers are trapped in a dilemma of optimizing model accuracy by training and fine-tuning models for each individual edge device while keeping the training GPU-hours tractable. In this paper, we propose Omni-sparsity DNN, where a single neural network can be pruned to generate optimized model for a large range of model sizes. We develop training strategies for Omni-sparsity DNN that allows it to find models along the Pareto front of word-error-rate (WER) vs model size while keeping the training GPU-hours to no more than that of training one singular model. We demonstrate the Omni-sparsity DNN with streaming E2E ASR models. Our results show great saving on training time and resources with similar or better accuracy on LibriSpeech compared to individually pruned sparse models: 2%-6.6% better WER on Test-other.

==> icassp/priorworks.tex <==
% \section{Prior Works}\label{sec:priorworks}

% Some past work explores the idea of sparse supernet for ASR model training. Wu et. al.~\cite{wu2021dynamic} developed dynamic sparsity for neural-network (DSNN) based speech models, as a framework to train a few speech models at pre-defined sparsity in one supernet. Different from our work, the DSNN applies a fixed number of pre-defined target sparsity level uniformly to each of the layers of the ASR models. It can not produce model with sparsity not pre-defined in the training process. In addition, it is not guaranteed that the DSNN-trained models would lie on the Pareto front of WER vs model size.

% Other works apply differentiable architecture search (Darts)~\cite{liu2019darts} to ASR models~\cite{liu2021improved, hu2021neural, shi2021dartsconformer} or end-to-end key word spotting models~\cite{zhang2020autokws}. In general, these work differ from our work in that they focus on varying layer operation type, layer width and sizes. 
% In~\cite{liu2021improved,shi2021dartsconformer}, the authors used Darts to search for different combinations of convolution, feed-forward network and multi-headed self attention blocks inside the conformation modules. Their work do not address model compression and the trade off between WER and model sizes. In addition, the Darts-based NAS utilizes validation loss, instead of the final model evaluation metrics (i.e. WER), to determine optimal architecture. 
